EDBooks: AI-Enhanced Interactive Narratives for Programming Education

Large Language Models (LLMs) have shown the potential to be valuable teaching tools, with the potential of giving every student a personalized tutor. However, one challenge with using LLMs to learn new concepts is that when learning a topic in an unfamiliar domain, it can be difficult to know what questions to ask. Further, language models do not always encourage "active learning" where students can test and assess their understanding. In this paper, we propose ways to combine large language models with "traditional" learning materials (like e-books) to give readers the benefits of working with LLMs (the ability to ask personally interesting questions and receive personalized answers) with the benefits of a traditional e-book (having a structure and content that is pedagogically sound). This work shows one way that LLMs have the potential to improve learning materials and make personalized programming education more accessible to a broader audience.

==> sections/8-Acknowledgments.tex <==
% We thank Lucy Ling and Jason Dominic for providing valuable feedback on the design of the \platform{} \ac{UI}.
% Michael Nebeling provided helpful feedback on the writing.

==> sections/A1-Task-Chapters.tex <==
\subsubsection{Task 1: \taskscheme{}}
The Scheme-related task (\taskscheme{}) consisted of four chapters:
\begin{itemize}
    \item \textbf{1 -- Introduction to Scheme} introduces history of Scheme and reasons to use Scheme.
    \item \textbf{2 -- Scheme Expressions} introduces concepts such as s-expression, prefix notation and using the \texttt{print} function in Scheme.
    \item \textbf{3 -- Basic Syntax of Scheme} covers syntax of Scheme, including atoms, lists, strings, adding comments, and using single quotation.
    \item \textbf{4 -- Functions} covers how to define functions, the \texttt{format} function, and the \texttt{newline} function.
\end{itemize}

\subsubsection{Task 2: \taskcache{}}
The caching-related task (\taskcache{}) consisted of five chapters:

\begin{itemize}
    \item \textbf{1 -- Introduction to Cache} introduces reasons to use caching.
    \item \textbf{2 -- Private Functions} covers importing libraries needed to implement caching in Python and file processing including reading and writing files.
    \item \textbf{3 -- Updating the Cache} covers how to add new data to cache dictionary.
    \item \textbf{4 -- Request URLs and Keys} explains making an HTTP request and creating unique key that will be used as the key value in cache dictionary.
    \item \textbf{5 -- Getting Cached Data} explains retrieving cached data after checking the whether it meets the condition.
\end{itemize}

==> sections/ZZ-OLDIntroduction.tex <==
Programming skills are in high demand across a variety of industries, which has led to surging interest in computing education in both traditional and non-traditional learning environments.
However, providing high-quality programming education at scale remains challenging~\cite{qian2017students}.
Traditional classrooms can offer effective teaching and support but often lack enough instructors for personalized experiences.
Non-traditional environments like online courses and \ac{SDL} can provide scalable instruction but may lack personalized guidance and practice.
There is a need for educational experiences that provide responsive guidance while enabling learner agency and exploration. 
This is especially important in domains like programming, which require active hands-on practice and feedback to build skills.
Prior approaches using passive mediums like books and videos have limitations in providing truly adaptive and interactive content tailored to diverse learners' needs.
Thus, the question that motivates this research is: \textbf{how can we enable high-quality, personalized interactive learning experiences that scale?}
We are particularly focused on \emph{asynchronous} programming education, which can include \ac{SDL} or assignments that are part of a traditional course.
% We also scope our focus to \emph{programming education}, which remains in high demand and presents unique challenges~\cite{qian2017students}.

Recently, the advent of \acp{LLM} such as ChatGPT has opened new possibilities for developing engaging and personalized educational content that can provide responsive guidance at scale~\cite{heaven2023chatgpt,lin2023exploring}.
\acp{LLM} can generate human-like text, engage in natural language conversations, and accurately respond to a wide variety of questions and requests.
However, one challenge with using open-ended \acp{LLM} to learn new concepts is that it can be difficult for students to know what questions to ask to effectively build understanding in an unfamiliar domain.
Although many \emph{task-oriented} \ac{LLM} extensions (such as chatbots for booking flights) can naturally elicit information from users (e.g., departure airport, destination, etc.), they do not have a way to ensure readers are given educational content.
Ideally, learners should have the flexibility to explore and ask questions on their own while achieving larger learning goals, which could be specified by instructors and field experts.
This highlights a key challenge: \textbf{how can we enable programming learners to benefit from interactive \acp{LLM} while aligning interactions with pedagogical goals?}

In this paper, we propose a platform for \emph{dialogic learning}~\cite{wegerif2006dialogic} to address these challenges.
Dialogic learning emphasizes interactive, learner-centered approaches where students actively co-construct knowledge.
Although dialogic education is primarily focused on synchronous, interactive educational experiences, the principles can also be applied to static educational content.
For example, Daniel Friedman authored a series of books that teach computing concepts through a dialog between a learner and an instructor~\cite{friedman1995little,friedman1995seasoned}.
However, \acp{LLM} may allow dialogic educational experiences to be interactive and scalable.
One of the key innovations of our work is in giving learners a way to interact with \acp{LLM} that is pedagogically-productive and open-ended.

\begin{figure}[t]
    \centering
    \begin{tikzpicture}
    \node[inner sep=0pt, draw=figureborder, line width=1pt, rounded corners=0pt] at (0,0) {\includegraphics[width=\textwidth]{figures/edbook_main.png}};
    \end{tikzpicture}
    \caption{A screenshot of a \platform{} page that describes the basics of Python modules.
    Readers learn through an interactive dialog (left column) that includes a natural language didactic dialog, multiple choice questions, and code writing questions.
    With \platform{}, readers work through this narrative over time.
    At any point in the narrative, they can also interact with a context-embedded \ac{LLM} for additional questions.
    These dialogs can also include larger code samples that are incrementally built and explained over the course of the narrative (right column).
    Deictic pointers (represented as blue lines) can link the narratives with specific parts of code.
    At the bottom of the leftmost column, the reader is given three options for how to proceed with the narrative: two pre-built questions (``is \texttt{random} a built-in module?'' and ``Could we call \texttt{import} inside of \texttt{rollDice}?'') and the option to query an \ac{LLM}.
    }
    \label{fig:edbook-main}
\end{figure}


We designed \textbf{\platform{}}\footnote{``\platform{}'' is short for \textbf{\underline{E}}lectronic \textbf{\underline{D}}ialogic \textbf{\underline{Book}}} a new platform for shareable, interactive educational content\footnote{Readers are invited to try an anonymized deployment of \platform{} at \url{https://edbook.net/}.}.
With \platform{}, content authors can write dialog trees---dialogs where messages can have multiple responses---that are aimed towards a learning goal.
These dialogs can involve number of `participants' but typically contain at least an instructor persona who guides readers through didactic dialog and a persona representing the reader.
They can contain interactive code-writing questions to give readers hands-on practice, multiple-choice questions to help readers assess their understanding, larger code samples that are incrementally built and explained over the course of the dialog, and multimedia, as Figure~\ref{fig:edbook-main} shows.
Readers can interact with a pre-made dialog tree or can self-explore through open-ended interactions with a context-informed \ac{LLM}.
Readers are guided towards the learning goals that were pre-set by the original author, which is represented by a `target' point in the dialog tree---typically a leaf node that represents the end of the dialog.

\textbf{Contributions:}
The key innovation of this work is in enabling dialogic learning experiences that are open-ended yet goal-aligned.
By doing this, we can guide students towards a learning goal while providing responsive guidance and reinforcing concepts through interactive practice.
To our knowledge, this represents the first system to combine these techniques for text-based programming education.

The key contributions of this work are:
\begin{itemize}
    \item The design of \platform{}, a platform for interactive dialogic narratives that integrate \acp{LLM} into programming education content.
    \item Techniques to align open-ended \ac{LLM} interactions with larger learning goals, enabling learner agency while meeting pedagogical objectives. 
    \item A representation for branched dialogs, code examples, and learner state that maintains readability and understandability for learners.
    \item A study evaluating learning outcomes and qualitative experiences using \platform{} for programming education.
\end{itemize}

The \platform{} platform also includes several additional features that are not entirely novel but that are complimentary to its design, including
(1) interactive quiz questions (including code-writing questions and multiple-choice questions) that help students assess their understanding of the material,
(2) the ability to incrementally build up and explain large code samples over the course of a narrative, and
(3) the ability for deictic code pointers to better tie narratives with the larger code samples they discuss.
Although these features are not novel independently, we show how they can be effectively integrated into the larger \platform{} platform and dialogic learning more generally.
% 
Overall, our results highlight the promise of dialogic learning with \acp{LLM} for increased engagement, agency, and flexible learning tools that scale.
% We also discuss challenges and propose future work for aligning agency with pedagogical goals.
% There are still many open questions about how to best integrate \acp{LLM} into education in a way that is ethical, aligned with students' long-term interests, and pedagogically sound.
